DynIBaR: Neural Dynamic Image-Based Rendering

We address the problem of synthesizing novel views from a monocular video depicting a complex dynamic scene. State-of-the-art methods based on temporally varying Neural Radiance Fields (aka dynamic NeRFs) have shown impressive results on this task. However, for long videos with complex object motions and uncontrolled camera trajectories, these methods can produce blurry or inaccurate renderings, hampering their use in real-world applications. Instead of encoding the entire dynamic scene within the weights of MLPs, we present a new approach that addresses these limitations by adopting a volumetric image-based rendering framework that synthesizes new viewpoints by aggregating features from nearby views in a scene-motion-aware manner. Our system retains the advantages of prior methods in its ability to model complex scenes and view-dependent effects, but also enables synthesizing photo-realistic novel views from long videos featuring complex scene dynamics with unconstrained camera trajectories. We demonstrate significant improvements over state-of-the-art methods on dynamic scene datasets, and also apply our approach to in-the-wild videos with challenging camera and object motion, where prior methods fail to produce high-quality renderings. Our project webpage is at dynibar.github.io.

==> alternate_method.tex <==

\newcommand{\itoj}{{i \rightarrow j}}
\newcommand{\jtok}{{j \rightarrow k}}
\newcommand{\itojtok}{{i \rightarrow j \rightarrow k}}

\newcommand{\static}{^\textrm{static}}
\newcommand{\dynamic}{^\textrm{dynamic}}
\newcommand{\full}{^\textrm{full}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\boot}{\hat{\mathbf{B}}}


\section{Dynamic Image-Based Rendering}
Given a monocular video of a dynamic scene, with frames $( I_1, I_2, \ldots, I_N )$ and known camera parameters $(\Camera_1, \Camera_2, \ldots, \Camera_N)$, our goal is to synthesize a novel viewpoint at any desired time within the video. As in many other approaches, we train per-video: first optimizing our models to reconstruct the input frames, and then using these models to render novel views.

Rather than encoding 3D color and density directly in the weights of an MLP as in recent dynamic NeRF methods, we integrate ideas from classical IBR techniques with a volumetric rendering framework. Compared to surface rendering, volumetric representations have been shown to better model complex scene geometry with view-dependent effects. 

The following sections introduce our methods for modeling scene motion (Sec.~\ref{sec:method_motion}), multi-view feature aggregation (Sec.~\ref{sec:method_aggregation}), and enforcing temporal consistency via \emph{cross-time rendering in motion-adjusted ray space} (Sec.~\ref{sec:method_crosstime}). 
Our full system combines a static model and a dynamic model to produce color at each pixel. Accurate scene factorization is achieved by bootstrapped using segmentation masks derived from a separately trained pair of simpler static and dynamic model through Bayesian learning technique. (Sec.~\ref{sec:method_full}). 

\subsection{Motion trajectories}
\label{sec:method_motion}
To understand which points in an image correspond to which points at nearby times, we require a model of scene motion. One approach used in previous work is to estimate a scene flow field that predicts the movement from one time to the next at each sampled 3D point~\cite{li2021neural,zhang2021consistent}. However, to predict such motion across multiple frames requires repeated queries to such a model for each 3D point and is not computationally feasible in our volumetric IBR framework. 

Instead, we represent motion using \emph{motion trajectory fields} with a \emph{learnable basis}. For a point $\Pos$ and time $i$, a MLP $\MLP$ gives the motion trajectory coefficients
\begin{equation}
\Coeff_i (\Pos) = \{\coeff^l_i (\Pos) \}_{l=1}^{L} = \MLP \left(\gamma(\Pos), \gamma(i) \right),
\end{equation}
where $\coeff^l_i \in \mathcal{R}^3$ are coefficients for the $(x, y, z)$ positions, and $\gamma$ is positional encoding with linearly increasing frequency.
We set number of frequency to be $16$ based on the assumption that scene motions tend to be low frequency.

The point at time $j$ corresponding to $\Pos$ at time $i$, written $\Pos_\itoj$, is then given by:
\begin{equation}
\Pos_\itoj = \Pos + \sum_{l=1}^{L} \left(\basis^l_j - \basis^l_i\right) \coeff^l_i (\Pos)
\label{eq:relative_displace}
\end{equation}
where the $\basis_i^l$ are the coefficients of a learnable basis $\Basis$ of 1D motion trajectories. With this representation, determining the 3D locations corresponding to a given point at all different times requires only a single MLP query.

We initialize $\Basis$ to a DCT basis as proposed by Wang~\etal~\cite{wang2021neural}, but also fine-tune it during optimisation: we observe that fine-tuning allows us to model a wider range of motions in real world scenarios, as shown in the third row of Fig.~\ref{fig:ablations}.

\subsection{Feature aggregation}
\label{sec:method_aggregation}
\begin{figure}[t]
\centering
  \includegraphics[width=1.0\columnwidth]{figures/overview_new-1.pdf} 
  \caption{\textbf{Motion-adjusted multi-view feature aggregation.} Given sampled location $\Pos$ on the target ray $\rayi$ at time $i$, we estimate its motion trajectory coefficients $\Coeff_i(\Pos)$, which determine the corresponding 3D points $\Pos_\itoj$ for nearby times $j$. These are projected into their corresponding source views and used to extract image features $\feature_j$ which are then aggregated and processed via the ray transformer $\RayTransformer$ to produce per-sample color and density $(\cc, \sigma)$, from which the target image $\colorRender_i$ is synthesized by volume rendering. \todo{Remove $\Gamma$ from figure if we use methods section without it.}}
\label{fig:overview_1}
\end{figure}

For synthesis we use features extracted from temporally nearby source views. To synthesize an image at time $i$, we first identify the source views $I_j$ within $r$ frames of $i$, that is, where $j \in \mathcal{N}(i) = [i - r, i + r]$. From each source view we extract a corresponding 2D feature map $F_j$ to form an input tuple $\{ I_j, \Camera_j, F_j \}$. \todo{How are features extracted?} 

Fig.~\ref{fig:overview_1} illustrates the process of rendering an output color $\colorRender_i(\rayi)$ for a target ray $\rayt$ at time $i$. We sample points $\Pos$ along the ray between $t_\textit{near}$ and $t_\textit{far}$, and for each such point we predict motion trajectories to determine the corresponding points $\Pos_\itoj$ for $j \in \mathcal{N}(i)$. Projecting each  $\Pos_\itoj$ into its source view $I_j$ and feature map $F_j$ using $\Camera_j$, we extract color and CNN feature vector $\feature_j$ at the corresponding 2D pixel location.

We then use the method of IBRNet~\cite{wang2021ibrnet} to turn these sets of features into color and density for each sample, first aggregating the $\feature_j$ into a single feature vector at each sample point $\Pos$, then processing the sequence of aggregated features and the ray direction to predict color and density for each sample. The output of this Ray Transformer process $\RayTransformer$ is a sequence of color and density pairs $(\colorStatic, \sigma)$ along the ray. To the formulation in IBRNet our method adds one additional input to $\RayTransformer$: an embedding $\gamma(i)$ of the time $i$. We then apply the standard NeRF volume rendering equations to obtain the pixel color $\colorRender_i(\rayi)$ from $(\colorStatic, \sigma)~$\cite{mildenhall2020nerf}.

\subsection{Cross-time rendering for temporal consistency}
\label{sec:method_crosstime}
\begin{figure}[t]
\centering
  \includegraphics[width=1.0\columnwidth]{figures/overview_new-2.pdf} 
  \caption{\textbf{Cross-time rendering.} To enforce temporal consistency, for each point $\Pos$ at time $i$ we first determine the corresponding point at a nearby time $j$, $\Pos_\itoj$. We then compute a second motion trajectory to map $\Pos_\itoj$ into nearby times and extract features from the resulting points $\Pos_\itojtok$ at times $k \in \mathcal{N}(j)$. Applying the ray transformer with time embedding $\gamma(j)$ and volume rendering, we obtain the pixel color $\colorRenderj$: a view at time $i$
  rendered `via' time $j$.
  \todo{notation in figure differs}}
\label{fig:overview_2}
\end{figure}

Training an image-based rendering model as described above has two notable problems. Firstly, as shown in prior work, temporal coherence is low as the model may learn a reconstruction of the scene that is disconnected in time~\cite{li2021neural, gao2021dynamic} (See examples in Fig.~\ref{fig:ablations}). Secondly, to optimize such a model, when rendering $I_i$ we must exclude features $\feature_i$ (i.e.~those features from the same time as the image being rendered), otherwise the network will learn a trivial solution and ignore all other inputs.
Therefore, we seek a method that can both enforce temporal consistency to build multi-view constraints, and allow the ray transformer $\RayTransformer$ to use features at the target time itself without becoming degenerate, since during novel view synthesis we would like to be able to use as much as information as possible to recover dynamic content.

To achieve these goals, we introduce \emph{cross-time rendering} in motion-adjusted ray space, shown in Fig.~\ref{fig:overview_2}. The idea is to render a view at time $i$ but \emph{via} some nearby time $j$. Thus, we randomly pick a nearby $j$ and instead of directly using sampled points $\Pos$ along target ray $\rayi$, we consider the motion-adjusted points $\Pos_\itoj$, and treat them as if they lie along a ray at time $j$---even though because of motion they may not lie in a straight line at all.

Specifically, having computed the motion-adjusted points $\Pos_\itoj$ we query the motion trajectory MLP again to predict the coefficients of further trajectories $\Coeff_j (\Pos_\itoj) = \MLP (\Pos_\itoj, \gamma(j))$, and use these to compute the corresponding points $(\Pos_\itoj)_\jtok$ for $k$ in the temporal window $\mathcal{N}(j)$, using Eq.~\ref{eq:relative_displace}.
These new 3D correspondences are projected into their source views $I_k$ with camera parameters $\Camera_k$ to extract RGB color and local image features $\feature_k$, which are pooled and input to the ray transformer just as before, together with the time embedding $\gamma(j)$. The result is a sequence of colors and densities $\cc_\itoj$ and $\sigma_\itoj$ at time $j$, which can be composited as before to obtain the cross-time-rendered pixel color which we call $\colorRenderj$.

\begin{figure}[t]
\centering
  \includegraphics[width=1.0\columnwidth]{figures/evaluations-2.pdf} 
  \caption{\textbf{Qualitative Ablations.} From left to right, we compare a system (a) without temporal consistency, (b) aggregating features using scene flow fields, (c) representing motion trajectory with fixed DCT basis, (d) with our configurations. We show PSNR over regions of moving objects.  }
\label{fig:ablations}
\end{figure}


\subsection{Combining static and dynamic models}
\label{sec:method_full}
With only a dynamic model, we observe that aggregating features from source views within a small temporal window is not sufficient to fill in contents near image boundaries, and that inaccurate estimated non-zero scene motion of static scene content tends to cause temporal jittering in view synthesis. Therefore, we follow the ideas of NSFF~\cite{li2021neural}, and model the entire scene using two separate representations. Dynamic content $(\colori, \sigma_i)$ is represented with a time-varying model as above (using cross-time rendering during training). Static content $(\colorStatic\static, \sigma\static)$ is represented with a time-invariant model, which uses a ray transformer in the same way as the time-varying model but aggregates features sampled from nearby views without any motion adjustment (i.e. along epipolar lines), and without the additional time input to $\RayTransformer$.

The dynamic and static predictions are combined and rendered to a single output color $\colorRenderStatic\full$ using the method for combining static and transient models of NeRF-W~\cite{MartinBrualla2020NeRFIT}. Each model's color and density estimates can also be rendered separately, giving predictions $\colorRenderStatic\static$ for the static and $\colorRenderStatic\dynamic$ for the dynamic content, which we use in our losses.
\todo{Unfortunately writing out the equation for the combination correctly would take quite a lot of space, because it would involve introducing $\alpha$, $\delta$, $T$, from the NeRF equations. Is it ok to go without?)}

Some previous methods use a time-varying model to predict the content of the \emph{entire scene}, and then introduce an extra blending weight to blend the colors and density from the two representations during volume rendering~\cite{li2021neural, gao2021dynamic}. However in our method, as in NeRF-W, the blending weight is not necessary since the time-varying model only needs to output content for the dynamic parts of the scene~\cite{MartinBrualla2020NeRFIT}.

\paragraph{Motion segmentation with Hybrid IBR}
To encourage accurate scene decomposition, Gao$~\etal$~\cite{gao2021dynamic} adopt semantic segmentation masks, relying on the assumption that all moving objects are within candidate labels of semantic segmentation outputs, and that segmentation masks are always temporally accurate. We too use segmentation masks for decomposition, but we observe that these assumptions do not hold in real-world scenarios. Therefore we instead obtain segmentation masks using a hybrid IBR method that enables motion segmentation of dynamic scenes. Our idea is inspired by Bayesian learning strategy from recent work~\cite{casualsam2022}, but integrated into a volumetric IBR framework. 

In particular, before training our main models we jointly train two bootstrap models---one static and one dynamic---and use these to obtain motion segmentation masks $M_i$ which are used in training the full model.
The bootstrap static model predicts pixel color $\boot\static$ with a time-invariant version of our feature-aggregation described above, i.e., by volume-rendering along each ray through epipolar feature aggregation without any allowance for scene motion. The bootstrap dynamic model is a 2D encoder-decoder network $\AED$ which predicts opacity $\alpha_i$, confidence $\beta_i$, and RGB image color $\boot_i$ from an image frame:
\begin{equation}
\alpha_i, \beta_i, \boot_i\dynamic = \AED(I_i).
\end{equation}
The combined bootstrap image is composited pixelwise:
\begin{align}
\boot_i = \alpha_i \odot \boot_i\dynamic
    +  (1 - \alpha_i) \odot \boot\static
\end{align}

To segment moving objects, we treat photometric inconsistency caused by scene dynamics as the heteroscedastic aleatoric uncertainty, where we model the uncertainty with zero-mean Cauchy distribution. \todo{I have no idea what the preceding sentence means.}
By taking the negative log likelihood, the loss function is written as 
\begin{align}
    \mathcal{L}_{\text{seg}} = \sum_{\rayi}\log (\beta_i(\rayi) + \frac{|| \boot_i(\rayi) - \colorGTStatic(\rayi)||^2}
    {\beta_i(\rayi)})
\end{align}

After optimizing these bootstrap models we obtain the motion segmentation mask $M_i$ of each input image $I_i$ by thresholding $\alpha_i$ at $0.9$.
We show our estimated motion segmentation masks in Fig.~\ref{fig:render_decomposition}.
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{0.025cm}
    \setlength{\itemwidth}{2.73cm}
    \renewcommand{\arraystretch}{0.5}
    \hspace*{-\tabcolsep}\begin{tabular}{ccc}
            \includegraphics[width=\itemwidth]{figures/fg-bg/skateboarding/full.png} &
            \includegraphics[width=\itemwidth]{figures/fg-bg/skateboarding/fg.png} &
            \includegraphics[width=\itemwidth]{figures/fg-bg/skateboarding/bg.png} \\
            \includegraphics[width=\itemwidth]{figures/fg-bg/swing/full.png} &
            \includegraphics[width=\itemwidth]{figures/fg-bg/swing/fg.png} &
            \includegraphics[width=\itemwidth]{figures/fg-bg/swing/bg.png} \\
            \includegraphics[width=\itemwidth]{figures/fg-bg/umbrella/umbrella-full.png} &
            \includegraphics[width=\itemwidth]{figures/fg-bg/umbrella/umbrella-fg.png} &
            \includegraphics[width=\itemwidth]{figures/fg-bg/umbrella/umbrella-bg.png} \\
            \vphantom{I}\footnotesize Full rendering &
            \vphantom{I}\footnotesize Dynamic contents &
            \vphantom{I}\footnotesize Static contents
        \\
    \end{tabular}\vspace{-0.2cm}
    \caption{\textbf{Motion segmentation.} Scene decomposition through our Baysian learning based motion segmentation. Our approach is able to segment challenging scene dynamics such as moving shadow, swing, and waving bushes.}
    \label{fig:render_decomposition}
\end{figure}

\paragraph{Bootstrapping with segmentation mask}
Having obtained the segmentation masks $M_i$, we use them to bootstrap our main system with a similar approach to that of Omnimatte~\cite{lu2021omnimatte}, by applying a reconstruction loss on the time-variant model in dynamic regions, and on the time-invariant model in static regions:
\begin{align}
    \Lmask = &\sum_{\rayi} M_i (\rayi) \rho (\colorRenderStatic\static(\rayi), \colorGTStatic_i (\rayi)) \nonumber \\
    + &\sum_{\rayi} (1 - M_i(\rayi))  \rho (\colorRenderStatic\dynamic (\rayi), \colorGTStatic_i (\rayi))
\end{align}
where we perform morphological erosion and dilation operations on $M_i$ to obtain masks of dynamic and static regions respectively. \todo{So the equations are actually not correct?} We bootstrap the system with this masked reconstruction loss and decay the weights by 10 and 2 for dynamic and static parts respectively every 40K optimization steps.
\todo{What do 10 and 2 mean? A factor of 10?}

\subsection{Global spatial coordinate embedding}
To improve global spatial reasoning, we append a spatial coordinate embedding as an input to the ray transformer, in addition to the time embedding. 
In particular, for the time-invariant model, for every sampled point location $\Pos_i$, we 
concatenate each extracted local image feature with its corresponding (1) ray coordinate with respect to the target view, (2) ray coordinate with respect to the source view, and (3) 3D 
coordinate in the global reference frame~\cite{suhail2022light}. 
We use Pl\"{u}cker coordinates~\cite{jia2020plucker} to represent ray coordinates since it allows us to model arbitrary scene and camera geometry
without ambiguities or singularities.

For the time-varying model, recall that local image features are aggregated along curved rays during the optimization stage, but once optimization is complete, 
novel views are rendered by aggregating features along straight rays cast directly from the desired target view. 
As a result, we observe that concatenating the 3D coordinates of $\Pos_i$ or $\Pos_{i \rightarrow j}$ with the corresponding 2D image features as inputs to the ray transformer tends to impair view interpolation. 
Therefore, we concatenate the encoded global 3D 
coordinates of $\Pos_i$ with the features output from the multi-head attention layers in the ray transformer, in which multi-view feature aggregation is completed.

For all spatial coordinates, we apply a Fourier features--based positional encoding~\cite{mildenhall2020nerf, tancik2020fourier} with maximum frequency of 4.

\subsection{Regularization and Losses}
\label{sec:method_losses}
Our reconstruction loss $\LPho$ is a disocclusion-aware RGB photometric loss comparing $\colorRenderStatic\full(\rayi)$ with target pixel $\colorGTStatic_i(\rayi)$:
\begin{align}
    \Lpho = \sum_{\rayi} \sum_{j \in \mathcal{N}(i)} \hat{\mathbf{W}}_{j \rightarrow i} (\rayi) \rho (\colorGTStatic_i(\rayi), \colorRenderStatic\full(\rayi))
\end{align}
where $\rho$ is the generalized Charbonnier loss on RGB~\cite{charbonnier1994two} on RG and $\hat{\mathbf{W}}_{j \rightarrow i} (\rayi) $ is a motion disocculusion weight computed by the difference of accumulated alpha weights between time $i$ and $j$ to address motion disocclusion ambiguity as described by NSFF~\cite{li2021neural} (please see supplemental for more details). Note that when $j = i$, there is no scene motion induced displacement, and no disocculusion weight involved in the loss.

Photometric consistency alone is not sufficient to avoid bad local minima during optimization for monocular reconstruction~\cite{li2021neural, gao2021dynamic}. Therefore, we adopt regularizations used in previous approaches~\cite{barron2022mip, li2021neural, yoon2020novel, wu2022d}: $\Lreg = \Ldata + \LMT + \Lcp$. Here, $\Ldata$ is a data-driven term consisting of $L_1$ mono-depth and optical flow consistency priors from Zhang~\etal~\cite{zhang2021consistent} and RAFT~\cite{teed2020raft}; $\LMT$ is a motion-trajectory regularization term that encourages the estimated motion trajectory fields to be cycle consistent and spatio-temporally smooth; $\Lcp$ is a compactness prior that encourage scene decomposition and estimated geometry to be compact. We refer readers to the supplementary material for more details.

In summary, the total loss for optimizing our system is as follows:
\begin{align}
    \mathcal{L} & = \Lpho + \Lmask + \Lreg
\end{align}


